The Multifaceted Nature of Mentoring in OSS: Strategies, Qualities, and Ideal Outcomes

Mentorship in open source software (OSS) is a vital, multifaceted process that includes onboarding newcomers, fostering skill development, and enhancing community building. This study examines task-focused mentoring strategies that help mentees complete their tasks and the ideal personal qualities and outcomes of good mentorship in OSS communities. We conducted two surveys to gather contributor perceptions: the first survey, with 70 mentors, mapped 17 mentoring challenges to 21 strategies that help support mentees. The second survey, with 85 contributors, assessed the importance of personal qualities and ideal mentorship outcomes. Our findings not only provide actionable strategies to help mentees overcome challenges and become successful contributors but also guide current and future mentors and OSS communities in understanding the personal qualities that are the cornerstone of good mentorship and the outcomes that mentor-mentee pairs should aspire to achieve.

==> conclusion_future.tex <==
\section{Conclusion and Future Works}
